Sample-Conditioned Hypothesis Stability Sharpens Information-Theoretic Generalization Bounds

We present new information-theoretic generalization guarantees through the a novel construction of the "neighboring-hypothesis" matrix and a new family of stability notions termed sample-conditioned hypothesis (SCH) stability. Our approach yields sharper bounds that improve upon previous information-theoretic bounds in various learning scenarios. Notably, these bounds address the limitations of existing information-theoretic bounds in the context of stochastic convex optimization (SCO) problems, as explored in the recent work by Haghifam et al. (2023).

==> Discussions.tex <==
% \section{Concluding Remarks, Limitations and Future Works}
% Stability arguments are notorious for only providing in-expectation error
% bounds.


% \paragraph{Expressiveness of New CMI Notions Under Distribution-Free Setting}

%  Previous works \cite{steinke2020reasoning,haghifam2021towards,harutyunyan2021informationtheoretic,hellstrom2022a} have demonstrate that CMI framework is expressive enough to connect with VC theory for distribution-free learning setting. We now show the expressiveness of CMI quantities in this work.

%  \begin{thm}
%      Let $\mathcal{Z}=\mathcal{X}\times\{0,1\}$, and let $\mathcal{F}=\{f_w:\mathcal{X}\to\{0,1\}|w\in\mathcal{W}\}$ be a functional hypothesis class with finite VC dimension $d$. 
%      % Then, there exists an  $\mathcal{A}$ such that
%      % \[
%      % \frac{\beta_2}{n}\sum_{i=1}^n\sqrt{I(Z_i;U_i|\widetilde{W}_i)}\leq\beta_2\sqrt{\frac{(n+1)d\log{\frac{n}{2}}}{n}+\log{2}}.
%      % \]
%      Let $n>d+1$, for any $\beta_2$-stable algorithm, 
%      $
%      \frac{\beta_2}{n}\sum_{i=1}^n\sqrt{I(F_i,\bar{F}_i;U_i|\widetilde{Z}^+_i)}\leq\mathcal{O}\pr{\beta_2\pr{\sqrt{\frac{d\log{n/d}}{n}}+1}}.
%      % \beta_2\sqrt{\frac{(n+1)d\log{\frac{n}{2}}}{n}+\log{2}}.
%      $
%  \end{thm}

% \paragraph{SGD and SGLD}

% \paragraph{High-Probability Bound}

% \paragraph{Rate-Distortion}

% \paragraph{Other Limitations}
